Commutative Regular Languages with Product-Form Minimal Automata

We introduce a subclass of the commutative regular languages that is characterized by the property that the state set of the minimal deterministic automaton can be written as a certain Cartesian product. This class behaves much better with respect to the state complexity of the shuffle, for which we find the bound~$2nm$ if the input languages have state complexities $n$ and $m$, and the upward and downward closure and interior operations, for which we find the bound~$n$. In general, only the bounds $(2nm)^{|\Sigma|}$ and $n^{|\Sigma|}$ are known for these operations in the commutative case. We prove different characterizations of this class and present results to construct languages from this class. Lastly, in a slightly more general setting of partial commutativity, we introduce other, related, language classes and investigate the relations between them.

==> sc_shuffle_grp_lang.tex <==
Here, we give a sharp bound for the state complexity
of two commutative group languages.
However, in this case,  we do not express the bound in terms of the size
of recognizing input automata, but in terms of the index and period vectors
of the input languages. The result generalizes a corresponding result from~\cite{PighizziniS02}
for unary group languages to commutative group languages.

% todo group durch pure-group ersetzen!

\begin{toappendix}
For lower bound results, we also need the next results.

\begin{lemma}
\label{lem:lower_bound_sc}
 Let $\Sigma = \{a_1, \ldots, a_k\}$ and $(n_1, \ldots, n_k) \in \mathbb N_0^k$.
 Suppose for a commutative language $L \subseteq \Sigma^*$ we have
 \begin{enumerate}
 \item $\{ w \in \Sigma^* \mid \forall j \in \{1,\ldots, k\} : |w|_{a_j} \ge n_j \} \subseteq L$,
 \item $\{ w \in \Sigma^* \mid \exists j \in \{1,\ldots, k\} : |w|_{a_j} = \min\{n_j - 1,0\}  \} \cap L = \emptyset$.
 \end{enumerate}
 %\begin{multline*}
 %L \subseteq \{ w \in \Sigma^* \mid \exists j \in \{1,\ldots, k\} : |w|_{a_j} \ge n_j \}  \setminus \\
 %                     \{ w \in \Sigma^* \mid \forall j \in \{1,\ldots, k\} : |w|_{a_j} = \min\{n_j - 1,0\}  \},
 %\end{multline*}
 Then % todo notation sc einführen, hier vielleicht || || nutzen, oder stc_I für incomplete
 $
  \stc(L) = \prod_{j=1}^k (n_j + 1)
 $
 with index vector $(n_1, \ldots, n_k)$
 and period vector $(1,\ldots, 1)$.
\end{lemma}
\begin{proof}
 Set $\mathcal C = (\Sigma, [n_1+1] \times \ldots \times [n_k+1], \delta, (0,\ldots, 0), F)$
 with
 \begin{multline*}
  \delta((i_1, \ldots, i_{j-1}, i_j, i_{j+1}, \ldots, i_k), a_j) \\
   = (i_1, \ldots, i_{j-1}, (i_j + 1) \bmod (n_j+1), i_{j+1},\ldots, i_k).
 \end{multline*}
 and $F = \{ (\min\{ |w|_{a_1}, n_1 \}, \ldots, \min\{ |w|_{a_k}, n_k \}) \mid w \in L \}$.
 Then $L(\mathcal C) = L$.
 Let $(i_1, \ldots, i_k), (l_1, \ldots, l_k) \in [n_1+1] \times \ldots \times [n_k+1]$
 be distinct. Suppose, without loss of generality, $i_j > l_j$
 for some $j \in \{1,\ldots, k\}$.
 This implies $0 \le l_j < n_j$.
 Then
 $$
  \delta((l_1, \ldots, l_k), a_1^{n_1} \cdots a_{j-1}^{n_{j-1}} a_j^{n_j - 1 - l_j} a_{j+1}^{n_{j+1}} \cdots a_k^{n_k}) \notin F
 $$
 but
 $$ 
  \delta((i_1, \ldots, i_k), a_1^{n_1} \cdots a_{j-1}^{n_{j-1}} a_j^{n_j - 1 - l_j} a_{j+1}^{n_{j+1}} \cdots a_k^{n_k}) \in F
 $$
%  Then
%  $$
%   \delta( (l_1, \ldots, l_k), a_1^{\min\{ n_1 - 1 - l_1, 0\}} \cdots a_k^{\min\{ n_k - 1 - l_k, 0\}} ) \notin F.
%  $$
%  $$
%   \delta( (i_1, \ldots, i_k), a_1^{n_1-i_1} \cdots a_k^{n_k - i_k} ) \in F
%  $$
%  but
%  $$
%   \delta( (l_1, \ldots, l_k), a_1^{n_1-l_1} \cdots a_k^{n_k - l_k} ) \notin F.
%  $$
 Hence, all states are distinguishable and $\mathcal C$
 is isomorphic to the minimal automaton of $L$, which proves the claim. \qed
\end{proof}

% noch erweitern, dass "union-conform"
\begin{lemma}(Refining a result from \cite{PighizziniS02})
\label{lem:pighizziniS02_unary_group_lang_sc}
%  Let $U$ and $V$ be two unary group languages with periods $p$ and $q$.
%  Then $UV$ could be accepted by an automaton $\mathcal A = (\{a\}, Q, \delta, s_0, F)$
%  with index $\lcm(p,q) - 1$
%  and period $\gcd(p,q)$ 
 Let $\mathcal A = (\{a\}, Q, \delta, s_0, F)$
 and $\mathcal B = (\{a\}, P, \mu, t_0, E)$ be two unary automata
 with index zero and periods $p$ and $q$ respectively.
 Write $F = \{ f_1, \ldots, f_n\}$, $E = \{e_1, \ldots, e_m\}$.
 Then $L(\mathcal A) L(\mathcal B)$
 could be accepted by an automaton $\mathcal C = (\{a\}, R, \eta, r_0, T)$
 with index $\lcm(p,q) - 1$, period $\gcd(p,q)$ and 
 $T = \bigcup_{l=1}^n \bigcup_{h=1}^m T_{l,h}$ such
 that
 $$
  \{ w \mid \eta(r_0, w) \in T_{l, h} \} = \{ u \mid \delta(s_0, u) = f_l \} \cdot \{ v \mid \mu(t_0, v) = e_h\}
 $$
 for $l \in \{1,\ldots, n\}$ and $h \in \{1,\ldots, m\}$.
 %This result is optimal, i.e., there
 %exists unary languages $U$ and $V$ with minimal automata
 %that reach the stated bounds for the index
 %and period for the minimal automata of $U\cdot V$
 This result is optimal in the sense that
 there exists automata $\mathcal A$ and $\mathcal B$
 as above such that $\mathcal C$ is isomorphic
 to the minimal automaton of $L(\mathcal A)L(\mathcal B)$.
\end{lemma}
\begin{proof} The existence and optimality was stated in~\cite{PighizziniS02} as Theorem 8,
we only show the additional part about the final states.
With the notation from the statement,
set $\mathcal A_l = (\{a\}, Q, \delta, s_0, \{f_l\})$
and $\mathcal B_h = (\{a\}, Q, \mu, t_0, \{e_h\})$ 
for $l \in \{1,\ldots, n\}$ and $h \in \{1,\ldots,m\}$.
Then by~\cite{PighizziniS02} we have an automaton
with index $\lcm(p,q) - 1$
and period $\gcd(p,q)$ accepting $L(\mathcal A_l) \cdot L(\mathcal B_h)$
for $l \in \{1,\ldots, n\}$ and $h \in \{1,\ldots,m\}$.
As the index and period determines the form
of the automaton uniquely, we can suppose the only differing parts
of those automata for each $l \in \{1,\ldots, n\}$
and $h \in \{1,\ldots, m\}$ are the final states.
Hence, we can write $\mathcal C_{l,h} = (\{a\}, R, \eta, r_0, T_{l, h})$
where $R$, $\eta$ and the start state $r_0$ are independent of $l$ and $h$, and
$$
 L((\{a\}, R, \eta, r_0, T_{l, h})) = L(\mathcal A_l) L(\mathcal B_h).
$$
Set $T = \bigcup_{l = 1}^n \bigcup_{h = 1}^m T_{l,h}$, then
\begin{align*} 
 L((\{a\}, R, \eta, r_0, T))
  & =  \bigcup_{l = 1}^n \bigcup_{h = 1}^m L(\mathcal A_l) L(\mathcal B_h) \\
  & = \left( \bigcup_{l = 1}^n L(\mathcal A_l) \right) \cdot \left( \bigcup_{h = 1}^m L(\mathcal B_h) \right) \\
  & = L(\mathcal A) L(\mathcal B).
\end{align*}
This shows our claim. $\qed$
\end{proof}


\begin{lemma}(Combining results from \cite{Hoffmann20,DBLP:conf/cai/Hoffmann19})
\label{lem:unary_aut_compatible_with_union}
 Let $\Sigma = \{a_1,\ldots, a_k\}$ and $L \subseteq \Sigma^*$ be a commutative regular language
 with index vector $(i_1, \ldots, i_k)$
 and period vector $(p_1, \ldots, p_k)$.
 Then we can write
 $$
  L = \bigcup_{l=1}^n U_1^{(l)} \shuffle \ldots \shuffle U_k^{(l)}
 $$
 with unary languages $U_j^{(l)} \subseteq \{a_j\}^*$  for $j \in \{1,\ldots, k\}$.
 Furthermore, we can find unary automata $\mathcal A_j = (\{a_j\}, Q_j, \delta_j, s_j, F_j)$
 with indices $i_j$ and periods $p_j$ and
 with $F_j = \{ f_j^{(1)}, \ldots, f_j^{(n)} \}$
 such that for $l \in \{1,\ldots, n\}$
 $$
  U_j^{(l)} = \{ u \in \{a_j\}^* : \delta_j(u) = f_j^{(l)} \}
 $$
 and $|Q_j| = i_j + p_j$. Hence $L(\mathcal A_j) = \{ a_j^{|u|_{a_j}} \mid u \in L \} = \bigcup_{l=1}^n U_j^{l}$.
\end{lemma}
\begin{proof} 
We refer to~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20,GomezA08}
for the definition of the minimal commutative automaton.
We also use the same notation for the languages $U_j^{(l)}$
as used in~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}.
The first claim is stated as Corollary~2 in~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}.
Lemma 5 of~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}
states that we can derive from the minimal commutative automaton
a unary automaton with $i_j + p_j$ states such that
$U_j^{(l)}$ for $l \in \{1,\ldots, n\}$ is precisely the set of words
that lead this automaton into a single final state.
For each $U_j^{(l)}$ the automaton with $i_j + p_j$ states
is the same automaton. Hence, collecting in $F$ all the final
states corresponding to the $U_j^{(l)}$ gives the claim.
Note that we could have $U_j^{(l)} = U_j^{(l')}$
for distinct $l, l' \in \{1,\ldots, n\}$.
Also note that by definition, and as the minimal commutative automaton
is deterministic, if $U_j^{(l)} \ne U_j^{(l')}$, then 
$U_j^{(l)} \cap U_j^{(l')} = \emptyset$. \qed
\end{proof}
\end{toappendix}

 \begin{theoremrep}
   \label{thm:sc_comm_grp_lang}
     Let $\Sigma = \{a_1,\ldots, a_k\}$. 
     For commutative group languages $U, V \subseteq \Sigma^*$
     with period vectors $(p_1, \ldots, p_k)$
     and $(q_1, \ldots, q_k)$ their shuffle $U\shuffle V$
     has index vector $(i_1, \ldots, i_k)$ with $i_j = \lcm(p_j, q_j) - 1$ 
     for $j \in \{1,\ldots, k\}$
     %has index vector $(\lcm(p_1, q_1) - 1, \ldots, \lcm(p_k, q_k) - 1)$
     and period vector 
     $(\gcd(p_1, q_1), \ldots, \gcd(p_k, q_k))$. Hence, by Theorem~\ref{thm:sc_index_period},
     $$
      \stc(U\shuffle V) \le \prod_{j=1}^k ( \gcd(p_j, q_j) + \lcm(p_j, q_j) - 1).
     $$
     And this bound is sharp\footnote{I mention in passing that, for this result,
     it does not matter if we measure the state complexity in terms
     of complete or incomplete automata, as the input and result automata are always complete without
     a non-final sink state.}, i.e., there exist commutative group languages
     such that a minimal automaton accepting their shuffle reaches the bound.
    \end{theoremrep}
    \begin{proof}
 Write
 \begin{align*}
     U & = \bigcup_{l=1}^n U_1^{(l)} \shuffle \ldots \shuffle U_k^{(l)} \\
     V & = \bigcup_{h=1}^m V_1^{(h)} \shuffle \ldots \shuffle V_k^{(h)}
 \end{align*}
 with, for $j \in \{1,\ldots, k\}$, unary automata $\mathcal A_j = (\{a_j\}, Q_j, \delta_j, s_j, F_j)$
 and $\mathcal B_j = (\{a_j\}, P_j, \mu_j, t_j, E_j)$, $F_j = \{ f_j^{(l)} \mid l \in \{1,\ldots, n\} \}$
 and $E_j = \{ e_j^{(h)} \mid h \in \{1,\ldots, m\} \}$, with indices zero
 and periods $p_j$ and $q_j$ respectively,
 according to Lemma~\ref{lem:unary_aut_compatible_with_union}.
 Let $\mathcal C_j = (\{a_j\}, R_j, \eta_j, r_j, T_j)$
 with $T_j = \bigcup_{l=1}^n \bigcup_{h=1}^m T_j^{(l,h)}$
 be automata according to Lemma~\ref{lem:pighizziniS02_unary_group_lang_sc}
 such that
 \begin{equation}\label{eqn:concat_parts}
  \{ u \mid \eta_j(r_j, u) \in  T_j^{(l,h)} \} = U_j^{(l)} \cdot V_j^{(h)}
 \end{equation}
 for $l \in \{1,\ldots, n\}$ and $h \in \{1,\ldots, m\}$. 
 Hence, the indices and periods of these automata, as stated in Lemma~\ref{lem:pighizziniS02_unary_group_lang_sc},
 are precisely $\lcm(p_j, q_j) - 1$ and $\gcd(p_j, q_j)$.
 Define
 $$
  \mathcal C = (\Sigma, R_1 \times \ldots \times R_k, \eta, (r_1, \ldots, r_k), T)
 $$
 with
 $$
  T = \bigcup_{l=1}^n \bigcup_{h=1}^m T_1^{(l,h)} \times \ldots \times T_k^{(l,h)}
 $$
 and transition function $\delta((r_1, \ldots, r_j, \ldots, r_k), a_j) = (r_1, \ldots, \delta_j(r_j, a_j), \ldots, r_k)$
 for $(r_1, \ldots, r_j, \ldots, r_k) \in R_1 \times \ldots \times R_k$.
 By construction of $\mathcal C$ and Equation~\eqref{eqn:concat_parts}, we have
 $$
  \delta(u, (r_1, \ldots, r_k)) \in T_1^{(l,h)} \times \ldots \times T_k^{(l,h)}
   \Leftrightarrow u \in ( U_1^{(l)} V_1^{(h)} ) \shuffle \ldots \shuffle ( U_k^{(l)} V_k^{(h)} )
 $$
 for $l \in \{1,\ldots, n\}$ and $h \in \{1,\ldots, m\}$. Hence
 \begin{align*}
  L(\mathcal C) 
   & = \bigcup_{l=1}^n \bigcup_{h=1}^m ( U_1^{(l)} V_1^{(h)} ) \shuffle \ldots \shuffle ( U_k^{(l)} V_k^{(h)} ) \\
   & = \bigcup_{l=1}^n \bigcup_{h=1}^m  U_1^{(l)} \shuffle \ldots \shuffle U_k^{(l)} \shuffle V_1^{(l)} \shuffle \ldots \shuffle V_k^{(l)}\\
   & = \left( \bigcup_{l=1}^n  U_1^{(l)} \shuffle \ldots \shuffle U_k^{(l)} \right) \shuffle \left( \bigcup_{h=1}^m  V_1^{(l)} \shuffle \ldots \shuffle V_k^{(l)} \right) \\
   & = U \shuffle V
 \end{align*}
 as the shuffle operation is commutative and distributive over union and
 for unary languages shuffle and concatenation are the same operations.
 Now, we show that the bound is sharp.
 Let $p, q$ be two distinct prime numbers. Then, every number greater than $p\cdot q - (p + q) + 1$
 could be written in the form $ap + bq$ with $a,b \ge 0$, and this is the minimal number
 with this property, i.e., $pq - (p+q)$ could not be written in that way; see~\cite{PighizziniS02}.
 Set $V_j = a_j^{p-1}(a_j^p)^*$, $W_j = a_j^{q-1}(a_j^q)^*$
 and $U_j = \{ a_j^{p + q - 2 + ap + bq} \mid a,b \ge 0 \} = V_j W_j$.
 Then
 $$
  \stc(V_1 \shuffle \ldots \shuffle V_k) = p^k.
 $$
 For, the permutation automaton $\mathcal C = (\Sigma, [p]^k, \delta, (0,\ldots,0), \{ (p-2, \ldots, p-2) \})$
 with
 $$
  \delta( (i_1, \ldots, i_{j-1}, i_j, i_{j+1},\ldots, i_k), a_j )
   = (i_1, \ldots, i_{j-1}, (i_j + 1) \bmod p, i_{j+1}, \ldots, i_k)
 $$
 accepts $V_1 \shuffle \ldots \shuffle V_k$, and it is easy to see that if a language is accepted % vielleicht genauer,todo
 by a permutation automaton with a single final state, then this automaton is minimal.
 Similarly, $\stc(W_1 \shuffle \ldots \shuffle W_k) = q^k$.
 
 Set $n_j = pq - 1$ for $j \in \{1,\ldots, k\}$. Then the language
 \begin{multline*}
      L = U_1 \shuffle \ldots \shuffle U_k = (V_1 W_1) \shuffle \ldots \shuffle (W_1 W_k) \\ 
       = (V_1 \shuffle \ldots \shuffle V_k) \shuffle (W_1 \shuffle \ldots \shuffle W_K).
 \end{multline*}
 fulfills the prerequisites of Lemma~\ref{lem:lower_bound_sc} with $(n_1, \ldots, n_k)$,
 as for each $j \in \{1,\ldots k\}$ we have $a_j^{pq - 2} \notin U_j$ and
 $a_j^{pq-1}a_j^* \subseteq U_j$.
 Hence,
 $$
  \stc(L) = (pq)^{|\Sigma|} = (\gcd(p,q) + \lcm(p,q) - 1)^{|\Sigma|}
 $$
 and the bound given by the statement is attained. \qed 
\end{proof}

By definition of the period vector in terms of the Nerode right-congruence
classes, and as an recognizing permutation automaton
for a group language is complete, every entry $p_j$, $j \in \{1,\ldots, k\}$,
of the period vector is a lower bound for the size of a minimal recognizing automaton.
Furthermore, as for any two numbers $n,m > 0$
we always have $\gcd(n,m) + \lcm(n,m) - 1 \le nm$,
we can deduce the next bound in terms of the size of recognizing automata.
The result improves the general bound $(2nm)^{|\Sigma|}$ from~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}
for the shuffle of two commutative regular languages.


\begin{theorem}
 Let $U, V \subseteq \Sigma^*$ be commutative group languages
 recognized by automata with $n$ and $m$ states.
 Then, $U\shuffle V$ is recognizable by an automaton with at most $(nm)^{|\Sigma|}$
 many states.
\end{theorem}

We do not know if the last bound is sharp. 
% ne, todo lower bound mit einem zyklus -> sind quadratisch viele für binar
% We can give the following lower bound.
% Let $N > 0$ and define the commutative pure-group language
% \[
%  L = \bigshuffle_{a \in \Sigma} a^{N-1}(a^N)^*.
% \]
% Then, a minimal accepting permutation automaton has $N^{|\Sigma|}$



